NetOrchLLM: Mastering Wireless Network Orchestration with Large Language Models

The transition to 6G networks promises unprecedented advancements in wireless communication, with increased data rates, ultra-low latency, and enhanced capacity. However, the complexity of managing and optimizing these next-generation networks presents significant challenges. The advent of large language models (LLMs) has revolutionized various domains by leveraging their sophisticated natural language understanding capabilities. However, the practical application of LLMs in wireless network orchestration and management remains largely unexplored. Existing literature predominantly offers visionary perspectives without concrete implementations, leaving a significant gap in the field. To address this gap, this paper presents NETORCHLLM, a wireless NETwork ORCHestrator LLM framework that uses LLMs to seamlessly orchestrate diverse wireless-specific models from wireless communication communities using their language understanding and generation capabilities. A comprehensive framework is introduced, demonstrating the practical viability of our approach and showcasing how LLMs can be effectively harnessed to optimize dense network operations, manage dynamic environments, and improve overall network performance. NETORCHLLM bridges the theoretical aspirations of prior research with practical, actionable solutions, paving the way for future advancements in integrating generative AI technologies within the wireless communications sector.

==> table.tex <==
\begin{table*}[]
\caption{Comparison of LLM-based frameworks for wireless networks  literature.}\label{tab:comp}
\begin{tabular}{|
>{\columncolor[HTML]{EFEFEF}}c |c|
>{\columncolor[HTML]{FFCCC9}}c |
>{\columncolor[HTML]{FFCCC9}}c |
>{\columncolor[HTML]{FFCCC9}}c |
>{\columncolor[HTML]{FFCCC9}}c |
>{\columncolor[HTML]{FFCCC9}}c |}
\hline
\cellcolor[HTML]{C0C0C0}\textbf{Paper} & \cellcolor[HTML]{C0C0C0}\textbf{Tools}                                                          &
\cellcolor[HTML]{C0C0C0}\textbf{Query Tool}         & \cellcolor[HTML]{C0C0C0}\textbf{Large-Scale Problems} & \cellcolor[HTML]{C0C0C0}\textbf{Environmental-Awareness} & \cellcolor[HTML]{C0C0C0}\textbf{Dynamicity} & \cellcolor[HTML]{C0C0C0}\textbf{Hallucinations} \\ \hline
                          \cite{yilma2024telecomrag}    & RAG                                                                                                                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} \checkmark} & \faTimesCircle[regular]                                          & \faTimesCircle[regular]                                    & \faTimesCircle[regular]                                      & \cellcolor[HTML]{9AFF99} less susceptible                                   \\ \hline
                          
                            \cite{maatouk2023teleqna}  & Q\&A                                                                                   &\cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} \checkmark }                                  & \faTimesCircle[regular]                                          & \faTimesCircle[regular]                                    & \faTimesCircle[regular]                                     & susceptible                                  \\ \hline
                          \cite{zou2024telecomgpt,tarkoma2023ai}    & Telecom-Specific Tuning                                                                & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} \checkmark }                                 & \faTimesCircle[regular]                                          & \faTimesCircle[regular]                                    & \faTimesCircle[regular]                                     & \cellcolor[HTML]{9AFF99}  less susceptible                                  \\ \hline
                            \cite{shen2024large,zou2023wireless,jiang2024large}  & Multi-agent    & \cellcolor[HTML]{FFFC9E}Partially                  & \faTimesCircle[regular]                                          & \faTimesCircle[regular]                                    & \faTimesCircle[regular]                                     & susceptible                                   \\ \hline
                            \cite{shao2024wirelessllm,bariah2024large,6Gllm,xu2024large}  & Multi-Modal Fusion                                                                                                    & \checkmark                  & \faTimesCircle[regular]                                          & \cellcolor[HTML]{FFFC9E}Partially           & \faTimesCircle[regular]                                     & susceptible                                   \\ \hline
                            \cite{nazar2024enwar}    & RAG + Multi-Modal Fusion                                                                                                                     & \cellcolor[HTML]{9AFF99}\faTimesCircle[regular]   & \faTimesCircle[regular]                                          & \cellcolor[HTML]{9AFF99}\checkmark                                     & \faTimesCircle[regular]                                      & \cellcolor[HTML]{9AFF99} less susceptible                                  \\ \hline
Ours                          & \begin{tabular}[c]{@{}l@{}}RAG+ Wireless Repository+\\ Multi-Modal Fusion\end{tabular}           & \cellcolor[HTML]{9AFF99}\faTimesCircle[regular]                        & \cellcolor[HTML]{9AFF99}\checkmark                 & \cellcolor[HTML]{9AFF99}\checkmark           & \cellcolor[HTML]{9AFF99}\checkmark              & \cellcolor[HTML]{9AFF99} less susceptible           \\ \hline
\end{tabular}
\end{table*}
